Implementation of a Volume-of-Fluid Method in a Finite Element Code with Applications to Thermochemical Convection in a Density Stratified Fluid in the Earth's Mantle

We describe the implementation of a second-order accurate volume-of-fluid interface tracking algorithm in the open source finite element code ASPECT, which is designed to model convection in the Earth's mantle. This involves the solution of the incompressible Stokes equations coupled to an advection diffusion equation for the temperature, a Boussinesq approximation that governs the dependence of the density on the temperature, and an advection equation for a marker indicating the two initial density states. The volume-of-fluid method is fully parallelized and is integrated with the adaptive mesh refinement algorithm in ASPECT. We present the results of several standard interface tracking benchmarks in order to demonstrate the accuracy of the method as well as the results of several benchmarks commonly used in the computational mantle convection community. Finally, we present the results of computations with and without adaptive mesh refinement of a model problem involving thermochemical convection in a computationally stratified fluid designed to provide insight into how thermal plumes, that eventually reach the Earth's surface as ocean island basalts, originate at structures on the core-mantle boundary known as Large Low Shear wave Velocity Provinces.

==> LaTeX_FILES/FOR_JMRs_THESIS.tex <==
In the case of any interface capturing algorithm, we would expect any structure under such conditions to be diffused beyond recovery at, if not before, this point, while a non-conservative  interface tracking algorithm may result in behavior that, while distinct, would have a similar effect.
\begin{figure}[th!]
    \begin{center}
        \includegraphics[width=0.5\textwidth]{fold_flow_B_04_t_244e7.png}
        \caption{An example of an underresolved `fold' structure.
            This example is from the computation in
            Figure~\ref{FIG:B = 0.4 at t' = 1.97 WITH AMR} for $\mathrm{B}=0.4$ at $t'=1.97 \cdot 10^{-2}$; it is at the very center of the domain.
            The arrow glyphs depict the current velocity pattern.
        }
        \label{FIG:DISCUSSION FOLD EXAMPLE}
    \end{center}
\end{figure}
Another case of interest is produced at the locations where the centers of the full depth convection cells coincide with the borders of the stratified convection cells for
$\mathrm{B}$ values that are moderately stratified, in particular,
$0.3 \le \mathrm{B} \le 1.0$.
Here, close examination of the evolution of the interface structures,
especially on the AMR meshes, notes an initial stronger velocity vortex forming
thin fold structures at early times, as shown in
Figure~\ref{FIG:DISCUSSION FOLD EXAMPLE}.
Note that at the current time, the velocity pattern is similar to a standard
shear flow with a vertical offset to the horizontal shear locations, and
explains the originating flow pattern.
The later dynamics then elongate and thin said structures while also folding
them back on the rest of the fluid interface.
Once the width of this structure becomes sufficiently small; i.e.,
$\lesssim 4 \, h$, the loss of required assumptions, in particular that there is only one interface in any $3 \times 3$ reconstruction block, makes the reconstruction of
the interfaces unreliable.
Once the width has reached $\approx 2 \, h$, the center interface (labeled b in
the example in Figure~\ref{FIG:DISCUSSION FOLD EXAMPLE}) can only be resolved
if there is a cell boundary between the two interfaces, and the folded
structure may resolve into a single interface if subject to a number of common
velocity fields due to either a similar progression as noted earlier, or due to
effectively having the three interfaces enter the same cell.
A similar effect can be expected in any situation with a similar banding
structure to the fluid interface.
As the dynamics of interest to the analysis in
section~\ref{SUBSUBSECTION:GENERAL OBSERVATIONS} relate to the entirety of the
modeled domain and the effects of the discussed artifacts are minor fluid
displacements within this region which consists of less than $0.02\%$ of the
domain, the effects are sufficiently small as to not adversely effect the
accuracy of the simulation for the aspects of interest.
As above, this artifact is due to the VOF algorithm being able to retain the
structure of the interface only up to the point where the dynamics of the
system force it into an underresolved state, where the nature of the numerical
algorithm has a greater effect on the local behavior of the interface than do the dynamics of the exact solution of the problem.

